Towards Establishing Guaranteed Error for Learned Database Operations

Machine learning models have demonstrated substantial performance enhancements over non-learned alternatives in various fundamental data management operations, including indexing (locating items in an array), cardinality estimation (estimating the number of matching records in a database), and range-sum estimation (estimating aggregate attribute values for query-matched records). However, real-world systems frequently favor less efficient non-learned methods due to their ability to offer (worst-case) error guarantees - an aspect where learned approaches often fall short. The primary objective of these guarantees is to ensure system reliability, ensuring that the chosen approach consistently delivers the desired level of accuracy across all databases. In this paper, we embark on the first theoretical study of such guarantees for learned methods, presenting the necessary conditions for such guarantees to hold when using machine learning to perform indexing, cardinality estimation and range-sum estimation. Specifically, we present the first known lower bounds on the model size required to achieve the desired accuracy for these three key database operations. Our results bound the required model size for given average and worst-case errors in performing database operations, serving as the first theoretical guidelines governing how model size must change based on data size to be able to guarantee an accuracy level. More broadly, our established guarantees pave the way for the broader adoption and integration of learned models into real-world systems.

==> constant_model_size.tex <==
The next lemma formalizes this observation, showing that the error will, in fact, increase linearly with data size if model size is kept constant.  

\begin{lemma}\label{lemma:error_linear}
    Let $\hat{f}$ be any model of size at most $s$ bits. The worst case error of $\hat{f}$ when approximating a dataset of size $n$, denoted by $\epsilon_n$ is $\Omega(n)$. That is, there exist constants $n_s$ and $C_s>0$ so that for all $n$ larger than $n_s$, there exists a dataset of size $n$ such that $\epsilon_n\geq C_{s} n$.   
    %Assume our dataset $D$ is sampled i.i.d. from some distribution $\chi$ with c.d.f $F_{\chi}$. Let $\epsilon_n^s$ be the lowest achievable error for a model of size at most $s$ for a dataset of size $n$. Then for large enough datasets of size $n$ and $n'$, $\epsilon_{n'}^s\geq \frac{n'}{n}\epsilon_{n}^s$. %Let $\hat{f}$ be a model with the lowest representation size, $s$ when achieving error $\epsilon$ on a data set of size $n$.  Then, consider any other function approximation, $\hat{f}'$ of size at most $s$, that achieves error $\epsilon'$ for a data set of size $n'$. For large enough data sizes $n$ and $n'$, we have $\epsilon'\geq \frac{n_2}{n_1}\epsilon$
\end{lemma}

The above lemma implies that if one wants to be able to achieve a desired error, $\epsilon$, one has to increase the model size as data size increases. 

\subsection{Proof of Lemma~\ref{lemma:error_linear}}
The proof uses the probabilistic method to show the existence of such a dataset. 

From any data distribution with c.d.f. $F$, sample two i.i.d datasets of size $n$ and $n'$, where $n<n'$. Let $f$ and $f'$ be the query functions for the datasets of size $n$ and $n'$, respectively. For any $\epsilon$, and by DKW, we have that
$$
Pr(\normx{\frac{1}{n}f-F}_\infty>\epsilon) \leq 2e^{-2n\epsilon^2}
$$
and 
$$
Pr(\normx{\frac{1}{n'}f'-F}_\infty>\epsilon) \leq 2e^{-2n'\epsilon^2}
$$
%So that 
%$$
%Pr(\normx{\frac{1}{n}f-\frac{1}{n'}f'}_\infty\leq2\epsilon)\geq 1+ 4e^{-2(n+n')\epsilon^2}-2e^{-2n\epsilon^2}-2e^{-2n'\epsilon^2}
%$$
We will set $n$ (and therefore $n'$) and $\epsilon$ so that $2e^{-2n\epsilon^2}<1$ (and therefore $2e^{-2n'\epsilon^2}<1$). Therefore, there exist $f$ and $f'$ such that $\normx{\frac{1}{n'}f'-F}_\infty<\epsilon$ and $\normx{\frac{1}{n}f-F}_\infty<\epsilon$ and therefore $\normx{\frac{1}{n'}f'-\frac{1}{n}f}_\infty<2\epsilon$. Consider any such $f$ and $f'$. Let $\hat{f}^*$ be the model of size at most $s$ that achieves the lowest possible error when approximating $f$. 

Let $n$ be large enough so that $s$ bits is not sufficient for answering queries exactly, and all function approximations will incur error $\epsilon_s>0$. So we have $\normx{\hat{f}^*-f}\geq \epsilon_s>0$

%Note that $\normx{\hat{f}^*-f}>0$, because we are approximating a discrete function with a continuous function approximation with size $s$ bits. [NEEDS PROOF]

Let $\hat{f}$ be any model of size at most $s$ approximating $f'$. We show that $\frac{1}{n'}\normx{\hat{f}'-f'}\geq\frac{0.5}{n}\normx{\hat{f}^*-f}$. Let $C_{s, n}=\frac{0.5}{n}\normx{\hat{f}^*-f}$. Therefore,
$C_{s, n}n'\leq\normx{\hat{f}'-f'}$, which completes the proof.

For the purpose of contradiction, assume $\frac{1}{n'}\normx{\hat{f}'-f'}<\frac{0.5}{n}\normx{\hat{f}^*-f}$. This would imply, 
$$\normx{\frac{1}{n'}\hat{f}'-\frac{1}{n}f}_1\leq \normx{\frac{1}{n'}\hat{f}'-\frac{1}{n'}f'}_1+ \normx{\frac{1}{n'}f'-\frac{1}{n}f}_1< \normx{\frac{1}{n'}f'-\frac{1}{n}f}_1+\frac{0.5}{n}\normx{\hat{f}^*-f}$$

Choosing $n$ s.t., $\normx{\frac{1}{n'}f'-\frac{1}{n}f}_1 \leq \frac{0.5}{n}\epsilon_s \leq \frac{0.5}{n}\normx{\hat{f}^*-f}$ proves the result

Choosing $\epsilon''< \frac{\epsilon-\epsilon'}{2}$
Which is a contradiction. 

We also need to ensure that $\sqrt{\frac{\ln(2)}{2n}}<\epsilon''$. Thus, choose $n$ so that $\sqrt{\frac{\ln(2)}{2n}}< \frac{\epsilon_s}{4}<\frac{\epsilon}{4}<\frac{\epsilon-\epsilon'}{2}$

\qed

==> incorrect_ce_1d.tex <==
Let $d=1$, and for any dataset $D\in \mathcal{D}$, let $f_D(q, r)=|\{p\in D, q \leq p\leq r+q\}|$. Let $\mathcal{F}=\{f_D, \forall D\in \mathcal{D}\}$. We are concerned with the metric entropy of the set $\mathcal{F}$ under different metrics, specifically, $\normx{.}_{1}$ and $\normx{.}_{\infty}$ norms. Denote by $\mathds{M}(\mathcal{F}, \normx{.}, \epsilon)$ the packing number of the set $\mathcal{F}$ and by $\mathds{N}(\mathcal{F}, \normx{.}, \epsilon)$ it's covering number.



\begin{lemma}
    Let $D_1$ and $D_2$ be written as an $n$-dimensional vector in sorted order. For a fixed $r$, $\normx{f_{D_1}(., r)-f_{D_2}(., r)}_1=\normx{D_1-D_2}_{1, r}$, where $\normx{D_1-D_2}_{1, r}=2\sum_i\min\{|D_1[i]-D_2[i]|, r\}$.
\end{lemma}

\begin{lemma}
    Let $D_1$ and $D_2$ be written as an $n$-dimensional vector in sorted order. $\normx{D_1-D_2}_{1}\leq \normx{f_{D_1}-f_{D_2}}_1\leq 2\normx{D_1-D_2}_{1}$
\end{lemma}

\textit{Proof}. We have 
\begin{align*}
 \normx{f_{D_1}-f_{D_2}}_1&=\int_r\int_q|f_{D_1}(q, r)-f_{D_2}(q, r)|\\
 &=\int_r 2\sum_i\min\{|D_1[i]-D_2[i]|, r\}   \\
 &=2\sum_i\int_r \min\{|D_1[i]-D_2[i]|, r\}   \\
 &=2\sum_i(\int_{r<|D_1[i]-D_2[i]|} r + \int_{r\geq|D_1[i]-D_2[i]|} |D_1[i]-D_2[i]|)\\
&= 2\sum_i(\frac{|D_1[i]-D_2[i]|^2}{2}+(|D_1[i]-D_2[i]|)(1-|D_1[i]-D_2[i]|))\\
&= 2\sum_i(|D_1[i]-D_2[i]|-\frac{|D_1[i]-D_2[i]|^2}{2})
\end{align*}

Therefore $\normx{f_{D_1}-f_{D_2}}_1\leq 2\normx{D_1-D_2}$. Furthermore, $|D_1[i]-D_2[i]|^2\leq |D_1[i]-D_2[i]|$ so that $$|D_1[i]-D_2[i]|-\frac{|D_1[i]-D_2[i]|^2}{2}\geq |D_1[i]-D_2[i]|-\frac{|D_1[i]-D_2[i]|}{2}=\frac{|D_1[i]-D_2[i]|}{2}.$$

As such, we have $\normx{f_{D_1}-f_{D_2}}_1\geq \normx{D_1-D_2}$


==> partitioning_theorem.tex <==
COULD ALSO BE INTERESTING TO SHOW RESULTS ON WHEN PARTIONING HELPS BASED ON COMPOSTABILITY OF THE QUERY FUNCTION

\begin{theorem}
    Consider the class, $\mathcal{F}$, of function approximators that partition the space into $k$ independent partitions and approximate each partition with a function approximator of size at most $s$, where $s$ is a constant independent of data size. Then to be able to achieve any error $\epsilon$, $k$ has to be $\Omega(n)$. That is, for any $\epsilon$, there exists a dataset, $D$, of size $n>n_\epsilon$, and constants $n_\epsilon$ and $C_\epsilon$ such that all function approximators in $\mathcal{F}$ that achieve error at most $\epsilon$ on $D$ will have at least $C_\epsilon n$ number of pieces.
\end{theorem}

NEED TO MAKE AN ASSUMPTION ABOUT THE QUERIES, THAT BREAKING THEM DOWN DOESN"T MAKE THE EASIER. E.G., A COMPOSTABLE QUERY FUNCTION

%Let $\hat{f}^*_{n, \epsilon}$ be a function approximation with the least number of pieces, $k$, to approximate a query function for a dataset of size $n$, with $\frac{n}{2}$ elements in [0, 0.5] and $\frac{n}{2}$ elements in [0.5, 1].  

%Consider half of the space with the largest number of pieces, $k'$. So $k'\geq \frac{k}{2}$. Then for all functions in $\mathcal{F}$ approximating the query function over $[0.5, 1]$, they must have at least $k'$ number of pieces. [THE ERROR WE DON"T KNOW]


Note that for any $\epsilon$, there exists a dataset of size $n$ that the best model achieves error at most $\epsilon$ with $k$ pieces, $k\geq 1$. Let the query function for this dataset be $f$


Let $\hat{f}^*_{n, \epsilon}$ be a function approximation with the least number of pieces, $k$, to approximate a query function for a dataset of size $n$.

Now for any $n'>n$, set $i=\frac{n'}{n}$, consider this dataset, $D_n$ whose elements are in $[0, 1]$. Create the dataset $D_n^{n'}=\cup_\{0\leq j< i\}(D_n/i+ \frac{j}{i})$. We argue that any function approximation of this dataset with error at most $\epsilon$ has to have at least $ik$ number of pieces.

For the purpose of contradiction, assume there exists a function approximator $\hat{f}$ with fewer than $ik$ pieces that approximates the query function to error at most $\epsilon$. Let this function approximator over the domain $[\frac{j}{i}, \frac{j+1}{i}]$ be $\hat{f}^j$ and let the query function over the domain be $f^j$. Observe that $f_n(x)=f^j(\frac{x}{i}+\frac{j}{i})-j\times n$. Similarly, $\hat{f}^j_n=\hat{f}^j(\frac{x}{i}+\frac{j}{i})-j\times n$ is an approximation to $f_n(x)$. Note that $\normx{f_n(x)-\hat{f}^j_n}=\normx{f^j(\frac{x}{i}+\frac{j}{i})-\hat{f}^j(\frac{x}{i}+\frac{j}{i})}=\int_0^1|f^j(\frac{x}{i}+\frac{j}{i})-\hat{f}^j(\frac{x}{i}+\frac{j}{i})|=i\int_{\frac{j}{i}}^{\frac{j+1}{i}}|f^j(x)-\hat{f}^j(x)|= \epsilon^j$

We have that $\normx{f-\hat{f}}=\frac{1}{i}\sum_j\epsilon^j\leq \epsilon$

Furthermore, let the number of pieces of $\hat{f}$ in $[\frac{j}{i}, \frac{j+1}{i}]$ be $k^j$, and let the set of partition points in that interval be $P^{j}$. %Note that $k'\geq\sum_{0\leq j< i}k^j-(i-1)$. 
Our goal is to show that $k'\geq ik$ and for the purpose of contradiction, assume $k'<ik$.

Using $P^j$, create the new partition set $P=\cup_ji(P^j-\frac{j}{i})$. Note that $|P|=k'-1$

Now for each partition induced by $P$, take the model from $\hat{f}_n^j$ with the lowest error for that partition. For this construction, the error is 
$$
\sum_{p\in P} \int |f^j(x)-\hat|
$$


This function approximation will have lower error than the original function, unless all $\hat{f}_n^j$ have the same error [PROOF]



 
%, with all elements in [0, 0.5] let $\hat{g}^*_{n, \epsilon}$ be the same but in $[0.5, 1]$. Both with error $\epsilon$ over the data range 

%Create a dataset $D'$ of size $2\times n$. Then, any function approximation of this function with error $\epsilon$ has to have at least $2k$ number of pieces. [Proof] 

Let $n'=i\times n$, and for any $n'$ find $i=\frac{n'}{n}$. Then, a model will have to have at least $\frac{n' k}{n}$ number of pieces on this dataset.  


==> range_ce.tex <==
\section{Impact of range on CE}\label{appx:impact_range_ce}
However, we show that indeed imposing a range on each attribute (i.e., having both a lower and an upper bound) does not change our bounds. Specifically, for answering a no-range cardinality estimation, defined in XXXX, the same bounds hold.

\begin{lemma}\label{lemma:ce_norange_bound}
    The same bounds as in Theorems~\ref{thm:ce_required_size} hold for no-range cardinality estimation.
\end{lemma}

The bounds on no-range cardinality estimation (i.e., Thoerem\ref{thm:ce_required_size}) can be seen as a strict generalization of Theorems~\ref{thm:index_required_size}, and we obtain the special case by setting $d=1$ CHECK IF THERE ARE CONDITIONS ON $d$ IN THE THEOREMS PROOFS. 

The results are of the similar form to the case of indexing, but with additionally showing the impact of dimensionality on the required size. We see that dimensionality amplifies the impact of both data size and error threshold, leading to larger required model sizes. XXXX SEE IF THIS TRUE, IT SEEMs to DEPENDS ON THE VALUES OF n and $\epsilon$ BUT PERHAPS THERE ARE CONDITIONS BASED ON THE PROOFS






\subsection{Proof of CE any D No range}

\textit{Proof}. Let $P=\{(\frac{i_1\epsilon}{k}, ..., \frac{i_d\epsilon}{k}), 0\leq i_1, ...,i_d\leq \frac{k}{2\epsilon}\}$ for an integer $k$ specified later. Let $P_1, P_2\subseteq P^{\frac{n}{k}}$, $P_1\neq P_2$, that is, $P_1$ and $P_2$ are datasets of size $\frac{n}{k}$ only containing points in $P$. Let $D_1$ be the dataset of size $n$, where each point in $P_1$ is repeated $k$ times, and similarly define $D_2$. Assume $D_1$ and $D_2$ differ on their $i$-th point and, w.l.o.g, its $d$-th dimension. We have that 


\begin{align*}
\normx{f_{D_1}-f_{D_2}}_1 &=\int_{q_1}...\int_{q_{d-1}} \normx{f_{D_1}(q_1, ..., q_{d-1}, .)-f_{D_2}(q_1, ..., q_{d-1}, .)}\\
&\geq \int_{0.5}^1...\int_{0.5}^1 \normx{f_{D_1}(q_1, ..., q_{d-1}, .)-f_{D_2}(q_1, ..., q_{d-1}, .)}\\
&= \normx{f_{D_1}(1, ..., 1, .)-f_{D_2}(1, ..., 1, .)}\int_{0.5}^1...\int_{0.5}^1 \\
&= \normx{f_{D_1}(1, ..., 1, .)-f_{D_2}(1, ..., 1, .)}0.5^{d-1} \\
&= \epsilon 0.5^{d-1} 
\end{align*}

The total number of distinct points subsets of $P$ are $C((\frac{k}{2\epsilon})^d+\frac{n}{k}, \frac{n}{k})$. Setting $k=\sqrt{n}$ we have $C((\frac{\sqrt{n}}{2\epsilon})^d+\sqrt{n}, \sqrt{n})\geq (\frac{\sqrt{n}^{d-1}}{(2\epsilon)^d}+1)^{\sqrt{n}}$. Substitute $\epsilon$ with $\epsilon2^{d-1}$ we have $(\frac{\sqrt{n}^{d-1}}{\epsilon^d2^{d^2}}+1)^{\sqrt{n}}$. \qed

\begin{lemma}
    Consider a 1-d database $D$ of size $n$ and another database $D'$ which is a subset of $D$ and does not contain points $p_1, .., p_k$. Then, $\normx{f_{D}-f_{D'}}_1=\sum_i (1-p_i)$.
\end{lemma}


\subsubsection{Proof tightness}
\textit{Proof}. Let $P=\{(\frac{i_1\epsilon}{n}, ..., \frac{i_d\epsilon}{n}), 0\leq i_1, ...,i_d\leq \frac{n}{\epsilon}\}$. Let $\bar{\mathcal{D}}=\{D\subseteq P^n\}$, be the set of all datasets of $n$ points where the points fall in $P$. Now for any $D\in \mathcal{D}$, we show that $\exists \bar{D}\in \bar{\mathcal{D}}$, s.t. $\normx{f_D-f_{\bar{D}}}_1\leq \epsilon$. Specifically, consider $\bar{D}$ such that $\bar{D}[i, j]=\lfloor \frac{n}{\epsilon}\times D[i, j]\rfloor\frac{\epsilon}{n}$ for all $i$. Such a $\bar{D}$ exists in $\bar{\mathcal{D}}$ as all its points belong to $P$. Furthermore, let $\hat{D}$ be a dataset such that $\hat{D}[i, j]=\bar{D}[i, j]$ for $j<d$ and $\hat{D}[i, d]=D[i, d]$. We have that 

\begin{align*}
&\normx{f_{D}-f_{\bar{D}}}_1 =\int_{q_1}...\int_{q_{d-1}} \normx{f_{D}(q_1, ..., q_{d-1}, .)-f_{\bar{D}}(q_1, ..., q_{d-1}, .)}\\
&\leq \int_{q_1}...\int_{q_{d-1}} \normx{f_{D}(q_1, ..., q_{d-1}, .)-f_{\hat{D}}(q_1, ..., q_{d-1}, .)}+\normx{f_{\bar{D}}(q_1, ..., q_{d-1}, .)-f_{\hat{D}}(q_1, ..., q_{d-1}, .)}
\end{align*}

Now note that the first $d-1$ dimensions of $\bar{D}$ and $\hat{D}$ are identical, so that applying the predicate on the first $d-1$ attributes of the datasets leads to the same filtered data points. Furthermore, the $d$-th dimension of the points differ by at most $\frac{\epsilon}{n}$,  

\begin{align*}
\normx{f_{D}-f_{\bar{D}}}_1 \leq \epsilon + \int_{q_1}...\int_{q_{d-1}} \normx{f_{D}(q_1, ..., q_{d-1}, .)-f_{\hat{D}}(q_1, ..., q_{d-1}, .)}
\end{align*}

Now recall that points in $D$ and $\hat{D}$ have identical last dimension, and thus, after applying the predicates $q_1$, ..., $q_{d-1}$, the difference between the remaining dataset is that one might have more points than the other. Let $\mathcal{I}_{q_1, ..., q_{d-1}}^j$ be an indicator function denoting when $j$-th data point matches exactly one of $D$ or $\hat{D}$ for the predicate defined by $q_1, ..., q_{d-1}$.  Therefore, we have $\normx{f_{D}(q_1, ..., q_{d-1}, .)-f_{\hat{D}}(q_1, ..., q_{d-1}, .)}=\sum_j\mathcal{I}_{q_1, ..., q_{d-1}}^j(1-D[j, d])$. Plugging this in, we obtain that 

\begin{align*}
\normx{f_{D}-f_{\bar{D}}}_1 &\leq \epsilon + \int_{q_1}...\int_{q_{d-1}} \sum_j\mathcal{I}_{q_1, ..., q_{d-1}}^j(1-D[j, d])\\
&=\epsilon + \sum_j(1-D[j, d])\int_{q_1}...\int_{q_{d-1}} \mathcal{I}_{q_1, ..., q_{d-1}}^j\\
&\leq \epsilon + \sum_j(1-D[j, d])\int_{q_1}...\int_{q_{d-2}} \frac{\epsilon}{n}\\
&\leq \epsilon + \sum_j\frac{\epsilon}{n}\\
&= 2\epsilon 
\end{align*}

The total number of distinct points subsets of $P$ are $C((\frac{n}{\epsilon})^d+n, n)\leq (e\frac{n^{d-1}}{\epsilon^d}+e)^n$. Setting $\epsilon$ to be $2\epsilon$ we obtain  $(\frac{e2^dn^{d-1}}{\epsilon^d}+e)^n$. \qed
